Measurement of Meson Resonance Production in $\pi^{-} + $C Interactions at SPS energies

We present measurements of $\rho^0$, $\omega$ and K$^{*0}$ spectra in $\pi^{-} + $C production interactions at 158 GeV/c and $\rho^0$ spectra at 350 GeV/c using the NA61/SHINE spectrometer at the CERN SPS. Spectra are presented as a function of the Feynman's variable $x_\text{F}$ in the range $0 < x_\text{F} < 1$ and $0 < x_\text{F} < 0.5$ for 158 GeV/c and 350 GeV/c respectively. Furthermore, we show comparisons with previous measurements and predictions of several hadronic interaction models. These measurements are essential for a better understanding of hadronic shower development and for improving the modeling of cosmic ray air showers.

==> authors-list.tex <==
\institute{
{National Nuclear Research Center, Baku, Azerbaijan}\label{inst0}
\and{Faculty of Physics, University of Sofia, Sofia, Bulgaria}\label{inst1}
\and{Ru{\dj}er Bo\v{s}kovi\'c Institute, Zagreb, Croatia}\label{inst2}
\and{LPNHE, University of Paris VI and VII, Paris, France}\label{inst3}
\and{Karlsruhe Institute of Technology, Karlsruhe, Germany}\label{inst4}
\and{Fachhochschule Frankfurt, Frankfurt, Germany}\label{inst5}
\and{University of Frankfurt, Frankfurt, Germany}\label{inst6}
\and{Wigner Research Centre for Physics of the Hungarian Academy of Sciences, Budapest, Hungary}\label{inst7}
\and{University of Bergen, Bergen, Norway}\label{inst8}
\and{Jan Kochanowski University in Kielce, Poland}\label{inst9}
\and{H. Niewodnicza\'nski Institute of Nuclear Physics of the
      Polish Academy of Sciences, Krak\'ow, Poland}\label{inst10}
\and{National Centre for Nuclear Research, Warsaw, Poland}\label{inst11}
\and{Jagiellonian University, Cracow, Poland}\label{inst12}
\and{University of Science and Technology, Cracow, Poland}\label{inst13}
\and{University of Silesia, Katowice, Poland}\label{inst14}
\and{University of Warsaw, Warsaw, Poland}\label{inst15}
\and{University of Wroc{\l}aw,  Wroc{\l}aw, Poland}\label{inst16}
\and{Warsaw University of Technology, Warsaw, Poland}\label{inst17}
\and{Institute for Nuclear Research, Moscow, Russia}\label{inst18}
\and{Joint Institute for Nuclear Research, Dubna, Russia}\label{inst19}
\and{National Research Nuclear University (Moscow Engineering Physics Institute), Moscow, Russia}\label{inst20}
\and{St. Petersburg State University, St. Petersburg, Russia}\label{inst21}
\and{University of Belgrade, Belgrade, Serbia}\label{inst22}
\and{University of Bern, Bern, Switzerland}\label{inst23}
\and{University of Geneva, Geneva, Switzerland}\label{inst24}
\and{Fermilab, Batavia, USA}\label{inst25}
\and{Los Alamos National Laboratory, Los Alamos, USA}\label{inst26}
\and{University of Colorado, Boulder, USA}\label{inst27}
\and{University of Pittsburgh, Pittsburgh, USA}\label{inst28}
}
\author{
{A.~Aduszkiewicz}\thanksref{inst15}
\and{Y.~Ali}\thanksref{inst12}
\and{E.V.~Andronov}\thanksref{inst21}
\and{T.~Anti\'ci\'c}\thanksref{inst2}
\and{B.~Baatar}\thanksref{inst19}
\and{M.~Baszczyk}\thanksref{inst13}
\and{S.~Bhosale}\thanksref{inst10}
\and{A.~Blondel}\thanksref{inst24}
\and{M.~Bogomilov}\thanksref{inst1}
\and{A.~Brandin}\thanksref{inst20}
\and{A.~Bravar}\thanksref{inst24}
\and{J.~Brzychczyk}\thanksref{inst12}
\and{S.A.~Bunyatov}\thanksref{inst19}
\and{O.~Busygina}\thanksref{inst18}
\and{H.~Cherif}\thanksref{inst6}
\and{M.~\'Cirkovi\'c}\thanksref{inst22}
\and{T.~Czopowicz}\thanksref{inst17}
\and{A.~Damyanova}\thanksref{inst24}
\and{N.~Davis}\thanksref{inst10}
\and{H.~Dembinski}\thanksref{inst4}
\and{M.~Deveaux}\thanksref{inst6}
\and{W.~Dominik}\thanksref{inst15}
\and{P.~Dorosz}\thanksref{inst13}
\and{J.~Dumarchez}\thanksref{inst3}
\and{R.~Engel}\thanksref{inst4}
\and{A.~Ereditato}\thanksref{inst23}
\and{S.~Faas}\thanksref{inst4}
\and{G.A.~Feofilov}\thanksref{inst21}
\and{Z.~Fodor}\thanksref{inst7, inst16}
\and{C.~Francois}\thanksref{inst23}
\and{X.~Garrido}\thanksref{inst4}
\and{A.~Garibov}\thanksref{inst0}
\and{M.~Ga\'zdzicki}\thanksref{inst6, inst9}
\and{M.~Golubeva}\thanksref{inst18}
\and{K.~Grebieszkow}\thanksref{inst17}
\and{F.~Guber}\thanksref{inst18}
\and{A.~Haesler}\thanksref{inst24}
\and{A.E.~Herv\'e}\thanksref{inst4}
\and{J.~Hylen}\thanksref{inst25}
\and{S.N.~Igolkin}\thanksref{inst21}
\and{A.~Ivashkin}\thanksref{inst18}
\and{S.R.~Johnson}\thanksref{inst27}
\and{K.~Kadija}\thanksref{inst2}
\and{E.~Kaptur}\thanksref{inst14}
\and{M.~Kie{\l}bowicz}\thanksref{inst10}
\and{V.A.~Kireyeu}\thanksref{inst19}
\and{V.~Klochkov}\thanksref{inst6}
\and{V.I.~Kolesnikov}\thanksref{inst19}
\and{D.~Kolev}\thanksref{inst1}
\and{A.~Korzenev}\thanksref{inst24}
\and{V.N.~Kovalenko}\thanksref{inst21}
\and{K.~Kowalik}\thanksref{inst11}
\and{S.~Kowalski}\thanksref{inst14}
\and{M.~Koziel}\thanksref{inst6}
\and{A.~Krasnoperov}\thanksref{inst19}
\and{W.~Kucewicz}\thanksref{inst13}
\and{M.~Kuich}\thanksref{inst15}
\and{A.~Kurepin}\thanksref{inst18}
\and{D.~Larsen}\thanksref{inst12}
\and{A.~L\'aszl\'o}\thanksref{inst7}
\and{T.V.~Lazareva}\thanksref{inst21}
\and{M.~Lewicki}\thanksref{inst16}
\and{B.~Lundberg}\thanksref{inst25}
\and{B.~{\L}ysakowski}\thanksref{inst14}
\and{V.V.~Lyubushkin}\thanksref{inst19}
\and{I.C.~Mari\c{s}}\thanksref{inst4}
\and{M.~Ma\'ckowiak-Paw{\l}owska}\thanksref{inst17}
\and{B.~Maksiak}\thanksref{inst17}
\and{A.I.~Malakhov}\thanksref{inst19}
\and{D.~Mani\'c}\thanksref{inst22}
\and{A.~Marchionni}\thanksref{inst25}
\and{A.~Marcinek}\thanksref{inst10}
\and{A.D.~Marino}\thanksref{inst27}
\and{K.~Marton}\thanksref{inst7}
\and{H.-J.~Mathes}\thanksref{inst4}
\and{T.~Matulewicz}\thanksref{inst15}
\and{V.~Matveev}\thanksref{inst19}
\and{G.L.~Melkumov}\thanksref{inst19}
\and{A.O.~Merzlaya}\thanksref{inst21}
\and{B.~Messerly}\thanksref{inst28}
\and{{\L}.~Mik}\thanksref{inst13}
\and{G.B.~Mills}\thanksref{inst26}
\and{S.~Morozov}\thanksref{inst18, inst20}
\and{S.~Mr\'owczy\'nski}\thanksref{inst9}
\and{Y.~Nagai}\thanksref{inst27}
\and{M.~Naskr\k{e}t}\thanksref{inst16}
\and{V.~Ozvenchuk}\thanksref{inst10}
\and{V.~Paolone}\thanksref{inst28}
\and{M.~Pavin}\thanksref{inst3, inst2}
\and{O.~Petukhov}\thanksref{inst18, inst20}
\and{C.~Pistillo}\thanksref{inst23}
\and{R.~P{\l}aneta}\thanksref{inst12}
\and{P.~Podlaski}\thanksref{inst15}
\and{B.A.~Popov}\thanksref{inst19, inst3}
\and{M.~Posiada{\l}a}\thanksref{inst15}
\and{S.~Pu{\l}awski}\thanksref{inst14}
\and{J.~Puzovi\'c}\thanksref{inst22}
\and{R.~Rameika}\thanksref{inst25}
\and{W.~Rauch}\thanksref{inst5}
\and{M.~Ravonel}\thanksref{inst24}
\and{R.~Renfordt}\thanksref{inst6}
\and{E.~Richter-W\k{a}s}\thanksref{inst12}
\and{D.~R\"ohrich}\thanksref{inst8}
\and{E.~Rondio}\thanksref{inst11}
\and{M.~Roth}\thanksref{inst4}
\and{B.T.~Rumberger}\thanksref{inst27}
\and{M.~Ruprecht}\thanksref{inst4}
\and{A.~Rustamov}\thanksref{inst0, inst6}
\and{M.~Rybczynski}\thanksref{inst9}
\and{A.~Rybicki}\thanksref{inst10}
\and{A.~Sadovsky}\thanksref{inst18}
\and{K.~Schmidt}\thanksref{inst14}
\and{I.~Selyuzhenkov}\thanksref{inst20}
\and{A.Yu.~Seryakov}\thanksref{inst21}
\and{P.~Seyboth}\thanksref{inst9}
\and{M.~S{\l}odkowski}\thanksref{inst17}
\and{A.~Snoch}\thanksref{inst6}
\and{P.~Staszel}\thanksref{inst12}
\and{G.~Stefanek}\thanksref{inst9}
\and{J.~Stepaniak}\thanksref{inst11}
\and{M.~Strikhanov}\thanksref{inst20}
\and{H.~Str\"obele}\thanksref{inst6}
\and{T.~\v{S}u\v{s}a}\thanksref{inst2}
\and{M.~Szuba}\thanksref{inst4}
\and{A.~Taranenko}\thanksref{inst20}
\and{A.~Tefelska}\thanksref{inst17}
\and{D.~Tefelski}\thanksref{inst17}
\and{V.~Tereshchenko}\thanksref{inst19}
\and{A.~Toia}\thanksref{inst6}
\and{R.~Tsenov}\thanksref{inst1}
\and{L.~Turko}\thanksref{inst16}
\and{R.~Ulrich}\thanksref{inst4}
\and{M.~Unger}\thanksref{inst4}
\and{F.F.~Valiev}\thanksref{inst21}
\and{D.~Veberi\v{c}}\thanksref{inst4}
\and{V.V.~Vechernin}\thanksref{inst21}
\and{M.~Walewski}\thanksref{inst15}
\and{A.~Wickremasinghe}\thanksref{inst28}
\and{C.~Wilkinson}\thanksref{inst23}
\and{Z.~W{\l}odarczyk}\thanksref{inst9}
\and{A.~Wojtaszek-Szwarc}\thanksref{inst9}
\and{O.~Wyszy\'nski}\thanksref{inst12}
\and{L.~Zambelli}\thanksref{inst3, inst}
\and{E.D.~Zimmerman}\thanksref{inst27}
\and{R.~Zwaska}\thanksref{inst25}
}

